Analytical Stellar Models of Neutron Stars in Teleparallel Gravity

In this paper, we developed three analytical models and obtained a new class of solutions describing compact stellar structures using the theory of teleparallel gravity. We consider the general anisotropic nature of stellar configurations and solve teleparallel gravity equations. In order to thoroughly analyze the various parameters of the stars, we developed three models by choosing various physically acceptable forms of metric potential $ e^{d(r)} $ and radial pressure $ p_r(r) $. We also analyze the impact of teleparallel gravity's parameters $ \beta $ and $ \beta_1 $ on the description of the stellar structures. We calculated model parameters such that models describing various observed neutron stars obey all physical conditions to be potentially stable and causal. By analyzing the impact of various parameters of teleparallel gravity on the description of anisotropic stellar structures, we found that three models developed in this paper can describe anisotropic neutron stars ranging from low density to high density. Finally, we obtain a quadratic Equation of State for each model describing various neutron stars, which can be utilized to find compositions of the stellar structures. It is very useful to find models that can exhibit quadratic EOS, since material compositions of real neutron stars and strange stars are found to exhibit quadratic EOS by various authors. Non linear $ f(T) $ model gives high deviation of EOS from quadratic behaviour, thus, in this paper we work with linear $ f(T) $ function by using diagonal tetrad to model realistic compact stars.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


